How to find a unicorn: a novel model-free, unsupervised anomaly detection method for time series

Recognition of anomalous events is a challenging but critical task in many scientific and industrial fields, especially when the properties of anomalies are unknown. In this paper, we introduce a new anomaly concept called "unicorn" or unique event and present a new, model-free, unsupervised detection algorithm to detect unicorns. The key component of the new algorithm is the Temporal Outlier Factor (TOF) to measure the uniqueness of events in continuous data sets from dynamic systems. The concept of unique events differs significantly from traditional outliers in many aspects: while repetitive outliers are no longer unique events, a unique event is not necessarily an outlier; it does not necessarily fall out from the distribution of normal activity. The performance of our algorithm was examined in recognizing unique events on different types of simulated data sets with anomalies and it was compared with the Local Outlier Factor (LOF) and discord discovery algorithms. TOF had superior performance compared to LOF and discord algorithms even in recognizing traditional outliers and it also recognized unique events that those did not. The benefits of the unicorn concept and the new detection method were illustrated by example data sets from very different scientific fields. Our algorithm successfully recognized unique events in those cases where they were already known such as the gravitational waves of a binary black hole merger on LIGO detector data and the signs of respiratory failure on ECG data series. Furthermore, unique events were found on the LIBOR data set of the last 30 years.

==> Figures/F1_prec_recall_table2.tex <==
\begin{tabular}{lcccc}
\toprule
dataset 	& $\,\,$	& 	TOF 	    &	LOF	 	& 	Discord	 \\
\cmidrule{1-5}
logmap-  &   M 		&	$121$	    &  $91$  	 	&	$21$	\\
tent	& $\mathrm{F}_1$& $\mathbf{0.869 \pm 0.055}$ & $0.640 \pm 0.130$ & $0.353 \pm 0.231$\\
		& precision	& $\mathbf{0.979 \pm 0.031}$ & $0.681 \pm 0.158$ & $0.835 \pm 0.305$\\
		& recall	& $\mathbf{0.797 \pm 0.069}$ & $0.777 \pm 0.175$	& $0.251 \pm 0.224$\\
logmap-  &   M 		&	$81$	    &  $1$  	 	&	$111$	\\
linear	& $\mathrm{F}_1$& $\mathbf{0.978 \pm 0.038}$ & $0.237 \pm 0.097$ & $0.528 \pm 0.398$\\
		& precision	& $\mathbf{0.978 \pm 0.053}$ & $0.138 \pm 0.062$	& $0.541 \pm 0.436$\\
		& recall	& $\mathbf{0.981 \pm 0.038}$ & $0.969 \pm 0.022$	& $0.58 \pm 0.428$\\
sim ECG- &   M 		&	$910$	    &  $1100$  	 	&	$1110$	\\
tachy	& $\mathrm{F}_1$& $\mathbf{0.834 \pm 0.094}$ & $0.452 \pm 0.102$ & $0.772 \pm 0.169$\\
		& precision	& $\mathbf{0.861 \pm 0.115}$ & $0.447 \pm 0.124$	& $0.784 \pm 0.264$\\
		& recall	& $0.815 \pm 0.091$ & $0.528 \pm 0.16$	& $\mathbf{0.868 \pm 0.16}$\\
randwalk &   M 		&	$51$	    &  $1$  	 	&	$221$	\\
linear	& $\mathrm{F}_1$& $\mathbf{0.977 \pm 0.018}$ & $0.209 \pm 0.092$ & $0.044 \pm 0.112$\\
		& precision	& $\mathbf{0.999 \pm 0.004}$ & $0.12 \pm 0.057$	& $0.039 \pm 0.101$\\
		& recall	& $\mathbf{0.956 \pm 0.033}$ & $0.954 \pm 0.039$	& $0.06 \pm 0.159$\\
\bottomrule
\end{tabular}



==> Figures/F1_prec_recall_table3.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-tent} \\
\cmidrule{1-5}
length (M) 	& $121$		 		&  $91$  	 	&	$21$		&  $137 \pm 94$ \\
$\mathrm{F}_1$	& $\mathbf{0.869 \pm 0.055}$ 	& $0.640 \pm 0.130$ 	& $0.353 \pm 0.231$	&  $0.002 \pm 0.016$ \\
precision	& $\mathbf{0.979 \pm 0.031}$ 	& $0.681 \pm 0.158$ 	& $0.835 \pm 0.305$	&  $0.002 \pm 0.014$\\
recall		& $\mathbf{0.797 \pm 0.069}$ 	& $0.777 \pm 0.175$ 	& $0.251 \pm 0.224$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-linear} \\
\cmidrule{1-5}
length (M) 	&	$81$			&  $1$  	 	&	$111$		& $147 \pm 91$ \\
$\mathrm{F}_1$	& $\mathbf{0.978 \pm 0.038}$ 	& $0.237 \pm 0.097$ 	& $0.528 \pm 0.398$	& $0.267 \pm 0.356$ \\
precision	& $\mathbf{0.978 \pm 0.053}$	& $0.138 \pm 0.062$ 	& $0.541 \pm 0.436$	& $0.22 \pm 0.358$ \\
recall		& $\mathbf{0.981 \pm 0.038}$	& $0.969 \pm 0.022$ 	& $0.58 \pm 0.428$	& $0.37 \pm 0.473$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{sim ECG-tachycardia} \\
\cmidrule{1-5}
length (M) 	&	$910$	    		&  $1100$  	 	&	$1110$		& $1128 \pm 1025$\\
$\mathrm{F}_1$	& $\mathbf{0.834 \pm 0.094}$ 	& $0.452 \pm 0.102$ 	& $0.772 \pm 0.169$	& $0.368 \pm 0.381$\\
precision	& $\mathbf{0.861 \pm 0.115}$ 	& $0.447 \pm 0.124$ 	& $0.784 \pm 0.264$	& $0.304 \pm 0.344$\\
recall		& $0.815 \pm 0.091$ 		& $0.528 \pm 0.16$	& $\mathbf{0.868 \pm 0.16}$ & $0.548 \pm 0.498$\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{random walk-linear} \\
\cmidrule{1-5}
length (M) 	&	$51$	   		&  $1$  	 	&	$221$		& $161 \pm 80$\\
$\mathrm{F}_1$	& $\mathbf{0.977 \pm 0.018}$ 	& $0.209 \pm 0.092$ 	& $0.044 \pm 0.112$	& $0.007 \pm 0.034$\\
precision	& $\mathbf{0.999 \pm 0.004}$ 	& $0.12 \pm 0.057$	& $0.039 \pm 0.101$	& $0.006 \pm 0.03$\\
recall	& $\mathbf{0.956 \pm 0.033}$ 	& $0.954 \pm 0.039$ 	& $0.06 \pm 0.159$	& $0.015 \pm 0.104$\\
\bottomrule
\end{tabular}



==> Figures/F1_prec_recall_table4.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-tent} \\
\cmidrule{1-5}
length (M) 	& $121$		 		&  $91$  	 	&	$91$		&  $137 \pm 94$ \\
$\mathrm{F}_1$	& $0.869 \pm 0.055$ 	& $0.640 \pm 0.130$ 	& $0.624 \pm 0.327$	&  $0.002 \pm 0.016$ \\
precision	& $0.979 \pm 0.031$ 	& $0.681 \pm 0.158$ 	& $0.72 \pm 0.385$	&  $0.002 \pm 0.014$\\
recall		& $0.797 \pm 0.069$ 	& $0.777 \pm 0.175$ 	& $0.586 \pm 0.3364$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-linear} \\
\cmidrule{1-5}
length (M) 	&	$81$			&  $1$  	 	&	$101$		& $147 \pm 91$ \\
$\mathrm{F}_1$	& $\mathbf{0.978} \pm 0.038$ 	& $0.237 \pm 0.097$ 	& $0.717 \pm 0.271$	& $0.267 \pm 0.356$ \\
precision	& $\mathbf{0.978} \pm 0.053$	& $0.138 \pm 0.062$ 	& $0.766 \pm 0.336$	& $0.22 \pm 0.358$ \\
recall		& $\mathbf{0.981} \pm 0.038$	& $0.969 \pm 0.022$ 	& $0.752 \pm 0.287$	& $0.37 \pm 0.473$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{sim ECG-tachycardia} \\
\cmidrule{1-5}
length (M) 	&	$910$	    		&  $1100$  	 	&	$1210$		& $1128 \pm 1025$\\
$\mathrm{F}_1$	& $\mathbf{0.834} \pm 0.094$ 	& $0.452 \pm 0.102$ 	& $0.765 \pm 0.176$	& $0.368 \pm 0.381$\\
precision	& $\mathbf{0.861} \pm 0.115$ 	& $0.447 \pm 0.124$ 	& $0.75 \pm 0.266$	& $0.304 \pm 0.344$\\
recall		& $0.815 \pm 0.091$ 		& $0.528 \pm 0.16$	& $\mathbf{0.894} \pm 0.14$ & $0.548 \pm 0.498$\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{random walk-linear} \\
\cmidrule{1-5}
length (M) 	&	$51$	   		&  $1$  	 	&	$141$		& $161 \pm 80$\\
$\mathrm{F}_1$	& $\mathbf{0.977} \pm 0.018$ 	& $0.209 \pm 0.092$ 	& $0.267 \pm 0.39$	& $0.007 \pm 0.034$\\
precision	& $\mathbf{0.999} \pm 0.004$ 	& $0.12 \pm 0.057$	& $0.284 \pm 0.423$	& $0.006 \pm 0.03$\\
recall		& $\mathbf{0.956} \pm 0.033$ 	& $0.954 \pm 0.039$ 	& $0.266 \pm 0.3859$	& $0.015 \pm 0.104$\\
\bottomrule
\end{tabular}



==> Figures/auc_table_v3.tex <==
\begin{tabular}{lcccccc}
\toprule\multicolumn{1}{c}{dataset} & $ $ & \multicolumn{2}{c}{TOF} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $ $ & $k$ &                AUC &  $ $ & $k$ &                AUC \\
\cmidrule{3-4} \cmidrule{6-7}logmap-tent    &   $\,$ &   2 &  $\mathbf{0.939 \pm 0.050}$ &  $\,$ &  42 &  $0.913 \pm 0.042$ \\
logmap-linear    &   $\,$ &   6 &  $\mathbf{0.994 \pm 0.007}$ &  $\,$ &  199 &  $0.847 \pm 0.213$ \\
sim ECG-tachy    &   $\,$ &   2 &  $\mathbf{0.931 \pm 0.039}$ &  $\,$ &  129 &  $0.815 \pm 0.056$ \\
randwalk-linear    &   $\,$ &   30 &  $\mathbf{0.988 \pm 0.014}$ &  $\,$ &  1 &  $0.572 \pm 0.015$ \\
\bottomrule
\end{tabular}

==> Figures/f1_table_v3.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - tent map} \\
\cmidrule{1-5}
length (M)    &   $121$  &    $91$  &    $91$   &  $137.06 \pm 93.68$ \\
$\mathrm{F}_1$	& $\mathbf{0.810 \pm 0.175}$ 	& $0.635 \pm 0.141$ & $0.624 \pm 0.329$	&  $0.002 \pm 0.016$ \\
precision    & $\mathbf{0.920 \pm 0.139}$ 	& $0.702 \pm 0.231$ & $0.720 \pm 0.387$	&  $0.002 \pm 0.014$ \\
recall	& $\mathbf{0.734 \pm 0.185}$ 	& $0.659 \pm 0.149$ & $0.586 \pm 0.337$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - linear} \\
\cmidrule{1-5}
length (M)    &   $81$  &    $91$  &    $101$   &  $146.56 \pm 91.17$ \\
$\mathrm{F}_1$	& $\mathbf{0.978 \pm 0.038}$ 	& $0.387 \pm 0.353$ & $0.717 \pm 0.273$	&  $0.267 \pm 0.358$ \\
precision    & $\mathbf{0.978 \pm 0.053}$ 	& $0.382 \pm 0.366$ & $0.766 \pm 0.332$	&  $0.220 \pm 0.308$ \\
recall	& $\mathbf{0.981 \pm 0.038}$ 	& $0.459 \pm 0.428$ & $0.752 \pm 0.289$	&  $0.370 \pm 0.473$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{sim ECG - tachycardia} \\
\cmidrule{1-5}
length (M)    &   $910$  &    $1110$  &    $1210$   &  $1128.04 \pm 1024.98$ \\
$\mathrm{F}_1$	& $\mathbf{0.834 \pm 0.094}$ 	& $0.428 \pm 0.092$ & $0.765 \pm 0.177$	&  $0.368 \pm 0.381$ \\
precision    & $\mathbf{0.861 \pm 0.115}$ 	& $0.425 \pm 0.119$ & $0.751 \pm 0.267$	&  $0.305 \pm 0.344$ \\
recall	& $0.815 \pm 0.091$ 	& $0.498 \pm 0.144$ & $\mathbf{0.894 \pm 0.141}$	&  $0.548 \pm 0.498$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{random walk - linear} \\
\cmidrule{1-5}
length (M)    &   $51$  &    $11$  &    $141$   &  $161.01 \pm 80.38$ \\
$\mathrm{F}_1$	& $\mathbf{0.977 \pm 0.018}$ 	& $0.024 \pm 0.024$ & $0.269 \pm 0.393$	&  $0.007 \pm 0.034$ \\
precision    & $\mathbf{0.999 \pm 0.004}$ 	& $0.127 \pm 0.092$ & $0.284 \pm 0.425$	&  $0.006 \pm 0.030$ \\
recall	& $\mathbf{0.956 \pm 0.033}$ 	& $0.014 \pm 0.015$ & $0.266 \pm 0.387$	&  $0.015 \pm 0.104$ \\
\bottomrule
\end{tabular}

==> Figures/my_auc_table.tex <==
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{dataset} & $\,\,$ & \multicolumn{2}{c}{TOF} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $\,\,$ & $k$ &                AUC &  $\,$ & $k$ &                AUC \\
\cmidrule{3-4} \cmidrule{6-7}
logmap tent     &   $\,$ &   2 &  $0.953 \pm 0.027$ &  $\,$ &  28 &  $0.928 \pm 0.075$ \\
logmap linear   &   $\,$ &   6 &  $0.996 \pm 0.004$ &  $\,$ &   1 &  $0.662 \pm 0.016$ \\
sim ECG  tachy  &   $\,$ &   3 &  $0.941 \pm 0.030$ &  $\,$ &  99 &  $0.834 \pm 0.053$ \\
randwalk linear &   $\,$ &  70 &  $0.993 \pm 0.007$ &  $\,$ &   1 &  $0.573 \pm 0.012$ \\
\bottomrule
\end{tabular}


==> Figures/my_auc_table_v2.tex <==
\begin{tabular}{lcccccc}
\toprule\multicolumn{1}{c}{dataset} & $ $ & \multicolumn{2}{c}{TOF} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $ $ & $k$ &                AUC &  $ $ & $k$ &                AUC \\
\cmidrule{3-4} \cmidrule{6-7}logmap-tent    &   $\,$ &   4 &  $0.909 \pm 0.087$ &  $\,$ &  42 &  $0.913 \pm 0.042$ \\
logmap-linear    &   $\,$ &   6 &  $0.994 \pm 0.007$ &  $\,$ &  199 &  $0.847 \pm 0.213$ \\
sim ECG-tachy    &   $\,$ &   4 &  $0.922 \pm 0.065$ &  $\,$ &  129 &  $0.815 \pm 0.056$ \\
randwalk-linear    &   $\,$ &   30 &  $0.988 \pm 0.014$ &  $\,$ &  17 &  $0.331 \pm 0.070$ \\
\bottomrule
\end{tabular}

==> Figures/my_f1_table.tex <==
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{c}{dataset} & $\,\,$ & \multicolumn{3}{c}{TOF} &  $\,$ & \multicolumn{3}{c}{LOF} \\
{} & $\,\,$ &     $\mathrm{F}_1$ &          precision &             recall &  $\,$ &     $\mathrm{F}_1$ &          precision &             recall \\
\cmidrule{3-5} \cmidrule{7-9}
logmap tent     &   $\,$ &  $0.869 \pm 0.055$ &  $0.979 \pm 0.031$ &  $0.797 \pm 0.069$ &  $\,$ &  $0.640 \pm 0.130$ &  $0.681 \pm 0.158$ &  $0.777 \pm 0.175$ \\
logmap linear   &   $\,$ &  $0.986 \pm 0.014$ &  $0.985 \pm 0.022$ &  $0.991 \pm 0.004$ &  $\,$ &  $0.009 \pm 0.002$ &  $0.009 \pm 0.000$ &  $0.009 \pm 0.004$ \\
sim ECG  tachy  &   $\,$ &  $0.816 \pm 0.095$ &  $0.818 \pm 0.129$ &  $0.868 \pm 0.052$ &  $\,$ &  $0.431 \pm 0.107$ &  $0.452 \pm 0.079$ &  $0.533 \pm 0.205$ \\
randwalk linear &   $\,$ &  $0.980 \pm 0.011$ &  $0.991 \pm 0.013$ &  $0.973 \pm 0.009$ &  $\,$ &  $0.014 \pm 0.010$ &  $0.019 \pm 0.000$ &  $0.012 \pm 0.013$ \\
\bottomrule
\end{tabular}


==> Figures/table_f1_table5.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - tent map} \\
\cmidrule{1-5}
length (M)    &   $121$  &    $91$  &    $91$   &  $137.06 \pm 93.68$ \\
$\mathrm{F}_1$	& $0.810 \pm 0.175$ 	& $0.635 \pm 0.141$ & $0.624 \pm 0.329$	&  $0.002 \pm 0.016$ \\
precision    & $0.920 \pm 0.139$ 	& $0.702 \pm 0.231$ & $0.720 \pm 0.387$	&  $0.002 \pm 0.014$ \\
recall	& $0.734 \pm 0.185$ 	& $0.659 \pm 0.149$ & $0.586 \pm 0.337$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - linear} \\
\cmidrule{1-5}
length (M)    &   $81$  &    $91$  &    $101$   &  $146.56 \pm 91.17$ \\
$\mathrm{F}_1$	& $0.978 \pm 0.038$ 	& $0.387 \pm 0.353$ & $0.717 \pm 0.273$	&  $0.267 \pm 0.358$ \\
precision    & $0.978 \pm 0.053$ 	& $0.382 \pm 0.366$ & $0.766 \pm 0.332$	&  $0.220 \pm 0.308$ \\
recall	& $0.981 \pm 0.038$ 	& $0.459 \pm 0.428$ & $0.752 \pm 0.289$	&  $0.370 \pm 0.473$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{sim ECG - tachycardia} \\
\cmidrule{1-5}
length (M)    &   $910$  &    $1110$  &    $1210$   &  $1128.04 \pm 1024.98$ \\
$\mathrm{F}_1$	& $0.834 \pm 0.094$ 	& $0.428 \pm 0.092$ & $0.765 \pm 0.177$	&  $0.368 \pm 0.381$ \\
precision    & $0.861 \pm 0.115$ 	& $0.425 \pm 0.119$ & $0.751 \pm 0.267$	&  $0.305 \pm 0.344$ \\
recall	& $0.815 \pm 0.091$ 	& $0.498 \pm 0.144$ & $0.894 \pm 0.141$	&  $0.548 \pm 0.498$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{random walk - linear} \\
\cmidrule{1-5}
length (M)    &   $51$  &    $21$  &    $141$   &  $161.01 \pm 80.38$ \\
$\mathrm{F}_1$	& $0.977 \pm 0.018$ 	& $0.040 \pm 0.026$ & $0.269 \pm 0.393$	&  $0.007 \pm 0.034$ \\
precision    & $0.999 \pm 0.004$ 	& $0.107 \pm 0.033$ & $0.284 \pm 0.425$	&  $0.006 \pm 0.030$ \\
recall	& $0.956 \pm 0.033$ 	& $0.027 \pm 0.023$ & $0.266 \pm 0.387$	&  $0.015 \pm 0.104$ \\
\bottomrule
\end{tabular}

==> TOF arXiv version2/Figures/Density_LOF_table.tex <==
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{dataset} & $\,\,$ & \multicolumn{2}{c}{Density} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $\,\,$ & $Normal$ &                Anomaly &  $\,$ & $Normal$ &                Anomaly \\
\cmidrule{3-4} \cmidrule{6-7}
logmap tent     &   $\,$ &   $95.759 \pm 12.070$ &  $11.606 \pm 1.146$ &  $\,$ & $1.039 \pm 0.010$ &  $3.424 \pm 1.990$ \\
logmap linear   &   $\,$ &   $95.190 \pm 9.305$ &  $97.413 \pm 51.289$ &  $\,$ &   $1.040 \pm 0.012$ &  $1.398 \pm 0.451$ \\
sim ECG  tachy  &   $\,$ &   $10146 \pm 2227$ &  $168.370 \pm 38.699$ &  $\,$ &  $1.106 \pm 0.022$ &  $1.264 \pm 0.227$ \\
randwalk linear &   $\,$ &  $197.919 \pm 3.866 $ &  $52590 \pm 61527$ &  $\,$ &   $1.623 \pm 0.661$ &  $1.872 \pm 0.920$ \\
\bottomrule
\end{tabular}


==> TOF arXiv version2/Figures/F1_prec_recall_table2.tex <==
\begin{tabular}{lcccc}
\toprule
dataset 	& $\,\,$	& 	TOF 	    &	LOF	 	& 	Discord	 \\
\cmidrule{1-5}
logmap-  &   M 		&	$121$	    &  $91$  	 	&	$21$	\\
tent	& $\mathrm{F}_1$& $\mathbf{0.869 \pm 0.055}$ & $0.640 \pm 0.130$ & $0.353 \pm 0.231$\\
		& precision	& $\mathbf{0.979 \pm 0.031}$ & $0.681 \pm 0.158$ & $0.835 \pm 0.305$\\
		& recall	& $\mathbf{0.797 \pm 0.069}$ & $0.777 \pm 0.175$	& $0.251 \pm 0.224$\\
logmap-  &   M 		&	$81$	    &  $1$  	 	&	$111$	\\
linear	& $\mathrm{F}_1$& $\mathbf{0.978 \pm 0.038}$ & $0.237 \pm 0.097$ & $0.528 \pm 0.398$\\
		& precision	& $\mathbf{0.978 \pm 0.053}$ & $0.138 \pm 0.062$	& $0.541 \pm 0.436$\\
		& recall	& $\mathbf{0.981 \pm 0.038}$ & $0.969 \pm 0.022$	& $0.58 \pm 0.428$\\
sim ECG- &   M 		&	$910$	    &  $1100$  	 	&	$1110$	\\
tachy	& $\mathrm{F}_1$& $\mathbf{0.834 \pm 0.094}$ & $0.452 \pm 0.102$ & $0.772 \pm 0.169$\\
		& precision	& $\mathbf{0.861 \pm 0.115}$ & $0.447 \pm 0.124$	& $0.784 \pm 0.264$\\
		& recall	& $0.815 \pm 0.091$ & $0.528 \pm 0.16$	& $\mathbf{0.868 \pm 0.16}$\\
randwalk &   M 		&	$51$	    &  $1$  	 	&	$221$	\\
linear	& $\mathrm{F}_1$& $\mathbf{0.977 \pm 0.018}$ & $0.209 \pm 0.092$ & $0.044 \pm 0.112$\\
		& precision	& $\mathbf{0.999 \pm 0.004}$ & $0.12 \pm 0.057$	& $0.039 \pm 0.101$\\
		& recall	& $\mathbf{0.956 \pm 0.033}$ & $0.954 \pm 0.039$	& $0.06 \pm 0.159$\\
\bottomrule
\end{tabular}



==> TOF arXiv version2/Figures/F1_prec_recall_table3.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-tent} \\
\cmidrule{1-5}
length (M) 	& $121$		 		&  $91$  	 	&	$21$		&  $137 \pm 94$ \\
$\mathrm{F}_1$	& $\mathbf{0.869 \pm 0.055}$ 	& $0.640 \pm 0.130$ 	& $0.353 \pm 0.231$	&  $0.002 \pm 0.016$ \\
precision	& $\mathbf{0.979 \pm 0.031}$ 	& $0.681 \pm 0.158$ 	& $0.835 \pm 0.305$	&  $0.002 \pm 0.014$\\
recall		& $\mathbf{0.797 \pm 0.069}$ 	& $0.777 \pm 0.175$ 	& $0.251 \pm 0.224$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-linear} \\
\cmidrule{1-5}
length (M) 	&	$81$			&  $1$  	 	&	$111$		& $147 \pm 91$ \\
$\mathrm{F}_1$	& $\mathbf{0.978 \pm 0.038}$ 	& $0.237 \pm 0.097$ 	& $0.528 \pm 0.398$	& $0.267 \pm 0.356$ \\
precision	& $\mathbf{0.978 \pm 0.053}$	& $0.138 \pm 0.062$ 	& $0.541 \pm 0.436$	& $0.22 \pm 0.358$ \\
recall		& $\mathbf{0.981 \pm 0.038}$	& $0.969 \pm 0.022$ 	& $0.58 \pm 0.428$	& $0.37 \pm 0.473$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{sim ECG-tachycardia} \\
\cmidrule{1-5}
length (M) 	&	$910$	    		&  $1100$  	 	&	$1110$		& $1128 \pm 1025$\\
$\mathrm{F}_1$	& $\mathbf{0.834 \pm 0.094}$ 	& $0.452 \pm 0.102$ 	& $0.772 \pm 0.169$	& $0.368 \pm 0.381$\\
precision	& $\mathbf{0.861 \pm 0.115}$ 	& $0.447 \pm 0.124$ 	& $0.784 \pm 0.264$	& $0.304 \pm 0.344$\\
recall		& $0.815 \pm 0.091$ 		& $0.528 \pm 0.16$	& $\mathbf{0.868 \pm 0.16}$ & $0.548 \pm 0.498$\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{random walk-linear} \\
\cmidrule{1-5}
length (M) 	&	$51$	   		&  $1$  	 	&	$221$		& $161 \pm 80$\\
$\mathrm{F}_1$	& $\mathbf{0.977 \pm 0.018}$ 	& $0.209 \pm 0.092$ 	& $0.044 \pm 0.112$	& $0.007 \pm 0.034$\\
precision	& $\mathbf{0.999 \pm 0.004}$ 	& $0.12 \pm 0.057$	& $0.039 \pm 0.101$	& $0.006 \pm 0.03$\\
recall	& $\mathbf{0.956 \pm 0.033}$ 	& $0.954 \pm 0.039$ 	& $0.06 \pm 0.159$	& $0.015 \pm 0.104$\\
\bottomrule
\end{tabular}



==> TOF arXiv version2/Figures/F1_prec_recall_table4.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-tent} \\
\cmidrule{1-5}
length (M) 	& $121$		 		&  $91$  	 	&	$91$		&  $137 \pm 94$ \\
$\mathrm{F}_1$	& $0.869 \pm 0.055$ 	& $0.640 \pm 0.130$ 	& $0.624 \pm 0.327$	&  $0.002 \pm 0.016$ \\
precision	& $0.979 \pm 0.031$ 	& $0.681 \pm 0.158$ 	& $0.72 \pm 0.385$	&  $0.002 \pm 0.014$\\
recall		& $0.797 \pm 0.069$ 	& $0.777 \pm 0.175$ 	& $0.586 \pm 0.3364$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{logmap-linear} \\
\cmidrule{1-5}
length (M) 	&	$81$			&  $1$  	 	&	$101$		& $147 \pm 91$ \\
$\mathrm{F}_1$	& $\mathbf{0.978} \pm 0.038$ 	& $0.237 \pm 0.097$ 	& $0.717 \pm 0.271$	& $0.267 \pm 0.356$ \\
precision	& $\mathbf{0.978} \pm 0.053$	& $0.138 \pm 0.062$ 	& $0.766 \pm 0.336$	& $0.22 \pm 0.358$ \\
recall		& $\mathbf{0.981} \pm 0.038$	& $0.969 \pm 0.022$ 	& $0.752 \pm 0.287$	& $0.37 \pm 0.473$ \\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{sim ECG-tachycardia} \\
\cmidrule{1-5}
length (M) 	&	$910$	    		&  $1100$  	 	&	$1210$		& $1128 \pm 1025$\\
$\mathrm{F}_1$	& $\mathbf{0.834} \pm 0.094$ 	& $0.452 \pm 0.102$ 	& $0.765 \pm 0.176$	& $0.368 \pm 0.381$\\
precision	& $\mathbf{0.861} \pm 0.115$ 	& $0.447 \pm 0.124$ 	& $0.75 \pm 0.266$	& $0.304 \pm 0.344$\\
recall		& $0.815 \pm 0.091$ 		& $0.528 \pm 0.16$	& $\mathbf{0.894} \pm 0.14$ & $0.548 \pm 0.498$\\
\cmidrule{1-5}
dataset  	& \multicolumn{4}{c}{random walk-linear} \\
\cmidrule{1-5}
length (M) 	&	$51$	   		&  $1$  	 	&	$141$		& $161 \pm 80$\\
$\mathrm{F}_1$	& $\mathbf{0.977} \pm 0.018$ 	& $0.209 \pm 0.092$ 	& $0.267 \pm 0.39$	& $0.007 \pm 0.034$\\
precision	& $\mathbf{0.999} \pm 0.004$ 	& $0.12 \pm 0.057$	& $0.284 \pm 0.423$	& $0.006 \pm 0.03$\\
recall		& $\mathbf{0.956} \pm 0.033$ 	& $0.954 \pm 0.039$ 	& $0.266 \pm 0.3859$	& $0.015 \pm 0.104$\\
\bottomrule
\end{tabular}



==> TOF arXiv version2/Figures/auc_table_v3.tex <==
\begin{tabular}{lcccccc}
\toprule\multicolumn{1}{c}{dataset} & $ $ & \multicolumn{2}{c}{TOF} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $ $ & $k$ &                AUC &  $ $ & $k$ &                AUC \\
\cmidrule{3-4} \cmidrule{6-7}logmap-tent    &   $\,$ &   2 &  $\mathbf{0.939 \pm 0.050}$ &  $\,$ &  42 &  $0.913 \pm 0.042$ \\
logmap-linear    &   $\,$ &   6 &  $\mathbf{0.994 \pm 0.007}$ &  $\,$ &  199 &  $0.847 \pm 0.213$ \\
sim ECG-tachy    &   $\,$ &   2 &  $\mathbf{0.931 \pm 0.039}$ &  $\,$ &  129 &  $0.815 \pm 0.056$ \\
randwalk-linear    &   $\,$ &   30 &  $\mathbf{0.988 \pm 0.014}$ &  $\,$ &  1 &  $0.572 \pm 0.015$ \\
\bottomrule
\end{tabular}

==> TOF arXiv version2/Figures/f1_table_v3.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - tent map} \\
\cmidrule{1-5}
length (M)    &   $121$  &    $91$  &    $91$   &  $137.06 \pm 93.68$ \\
$\mathrm{F}_1$	& $\mathbf{0.810 \pm 0.175}$ 	& $0.635 \pm 0.141$ & $0.624 \pm 0.329$	&  $0.002 \pm 0.016$ \\
precision    & $\mathbf{0.920 \pm 0.139}$ 	& $0.702 \pm 0.231$ & $0.720 \pm 0.387$	&  $0.002 \pm 0.014$ \\
recall	& $\mathbf{0.734 \pm 0.185}$ 	& $0.659 \pm 0.149$ & $0.586 \pm 0.337$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - linear} \\
\cmidrule{1-5}
length (M)    &   $81$  &    $91$  &    $101$   &  $146.56 \pm 91.17$ \\
$\mathrm{F}_1$	& $\mathbf{0.978 \pm 0.038}$ 	& $0.387 \pm 0.353$ & $0.717 \pm 0.273$	&  $0.267 \pm 0.358$ \\
precision    & $\mathbf{0.978 \pm 0.053}$ 	& $0.382 \pm 0.366$ & $0.766 \pm 0.332$	&  $0.220 \pm 0.308$ \\
recall	& $\mathbf{0.981 \pm 0.038}$ 	& $0.459 \pm 0.428$ & $0.752 \pm 0.289$	&  $0.370 \pm 0.473$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{sim ECG - tachycardia} \\
\cmidrule{1-5}
length (M)    &   $910$  &    $1110$  &    $1210$   &  $1128.04 \pm 1024.98$ \\
$\mathrm{F}_1$	& $\mathbf{0.834 \pm 0.094}$ 	& $0.428 \pm 0.092$ & $0.765 \pm 0.177$	&  $0.368 \pm 0.381$ \\
precision    & $\mathbf{0.861 \pm 0.115}$ 	& $0.425 \pm 0.119$ & $0.751 \pm 0.267$	&  $0.305 \pm 0.344$ \\
recall	& $0.815 \pm 0.091$ 	& $0.498 \pm 0.144$ & $\mathbf{0.894 \pm 0.141}$	&  $0.548 \pm 0.498$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{random walk - linear} \\
\cmidrule{1-5}
length (M)    &   $51$  &    $11$  &    $141$   &  $161.01 \pm 80.38$ \\
$\mathrm{F}_1$	& $\mathbf{0.977 \pm 0.018}$ 	& $0.024 \pm 0.024$ & $0.269 \pm 0.393$	&  $0.007 \pm 0.034$ \\
precision    & $\mathbf{0.999 \pm 0.004}$ 	& $0.127 \pm 0.092$ & $0.284 \pm 0.425$	&  $0.006 \pm 0.030$ \\
recall	& $\mathbf{0.956 \pm 0.033}$ 	& $0.014 \pm 0.015$ & $0.266 \pm 0.387$	&  $0.015 \pm 0.104$ \\
\bottomrule
\end{tabular}

==> TOF arXiv version2/Figures/my_auc_table.tex <==
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{dataset} & $\,\,$ & \multicolumn{2}{c}{TOF} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $\,\,$ & $k$ &                AUC &  $\,$ & $k$ &                AUC \\
\cmidrule{3-4} \cmidrule{6-7}
logmap tent     &   $\,$ &   2 &  $0.953 \pm 0.027$ &  $\,$ &  28 &  $0.928 \pm 0.075$ \\
logmap linear   &   $\,$ &   6 &  $0.996 \pm 0.004$ &  $\,$ &   1 &  $0.662 \pm 0.016$ \\
sim ECG  tachy  &   $\,$ &   3 &  $0.941 \pm 0.030$ &  $\,$ &  99 &  $0.834 \pm 0.053$ \\
randwalk linear &   $\,$ &  70 &  $0.993 \pm 0.007$ &  $\,$ &   1 &  $0.573 \pm 0.012$ \\
\bottomrule
\end{tabular}


==> TOF arXiv version2/Figures/my_auc_table_v2.tex <==
\begin{tabular}{lcccccc}
\toprule\multicolumn{1}{c}{dataset} & $ $ & \multicolumn{2}{c}{TOF} &  $\,$ & \multicolumn{2}{c}{LOF} \\
{} & $ $ & $k$ &                AUC &  $ $ & $k$ &                AUC \\
\cmidrule{3-4} \cmidrule{6-7}logmap-tent    &   $\,$ &   4 &  $0.909 \pm 0.087$ &  $\,$ &  42 &  $0.913 \pm 0.042$ \\
logmap-linear    &   $\,$ &   6 &  $0.994 \pm 0.007$ &  $\,$ &  199 &  $0.847 \pm 0.213$ \\
sim ECG-tachy    &   $\,$ &   4 &  $0.922 \pm 0.065$ &  $\,$ &  129 &  $0.815 \pm 0.056$ \\
randwalk-linear    &   $\,$ &   30 &  $0.988 \pm 0.014$ &  $\,$ &  17 &  $0.331 \pm 0.070$ \\
\bottomrule
\end{tabular}

==> TOF arXiv version2/Figures/my_f1_table.tex <==
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{c}{dataset} & $\,\,$ & \multicolumn{3}{c}{TOF} &  $\,$ & \multicolumn{3}{c}{LOF} \\
{} & $\,\,$ &     $\mathrm{F}_1$ &          precision &             recall &  $\,$ &     $\mathrm{F}_1$ &          precision &             recall \\
\cmidrule{3-5} \cmidrule{7-9}
logmap tent     &   $\,$ &  $0.869 \pm 0.055$ &  $0.979 \pm 0.031$ &  $0.797 \pm 0.069$ &  $\,$ &  $0.640 \pm 0.130$ &  $0.681 \pm 0.158$ &  $0.777 \pm 0.175$ \\
logmap linear   &   $\,$ &  $0.986 \pm 0.014$ &  $0.985 \pm 0.022$ &  $0.991 \pm 0.004$ &  $\,$ &  $0.009 \pm 0.002$ &  $0.009 \pm 0.000$ &  $0.009 \pm 0.004$ \\
sim ECG  tachy  &   $\,$ &  $0.816 \pm 0.095$ &  $0.818 \pm 0.129$ &  $0.868 \pm 0.052$ &  $\,$ &  $0.431 \pm 0.107$ &  $0.452 \pm 0.079$ &  $0.533 \pm 0.205$ \\
randwalk linear &   $\,$ &  $0.980 \pm 0.011$ &  $0.991 \pm 0.013$ &  $0.973 \pm 0.009$ &  $\,$ &  $0.014 \pm 0.010$ &  $0.019 \pm 0.000$ &  $0.012 \pm 0.013$ \\
\bottomrule
\end{tabular}


==> TOF arXiv version2/Figures/table_f1_table5.tex <==
\begin{tabular}{lcccc}
\toprule
method 	&	TOF 	    &	LOF	& 	Keogh	 &  Senin\\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - tent map} \\
\cmidrule{1-5}
length (M)    &   $121$  &    $91$  &    $91$   &  $137.06 \pm 93.68$ \\
$\mathrm{F}_1$	& $0.810 \pm 0.175$ 	& $0.635 \pm 0.141$ & $0.624 \pm 0.329$	&  $0.002 \pm 0.016$ \\
precision    & $0.920 \pm 0.139$ 	& $0.702 \pm 0.231$ & $0.720 \pm 0.387$	&  $0.002 \pm 0.014$ \\
recall	& $0.734 \pm 0.185$ 	& $0.659 \pm 0.149$ & $0.586 \pm 0.337$	&  $0.003 \pm 0.019$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{logistic map - linear} \\
\cmidrule{1-5}
length (M)    &   $81$  &    $91$  &    $101$   &  $146.56 \pm 91.17$ \\
$\mathrm{F}_1$	& $0.978 \pm 0.038$ 	& $0.387 \pm 0.353$ & $0.717 \pm 0.273$	&  $0.267 \pm 0.358$ \\
precision    & $0.978 \pm 0.053$ 	& $0.382 \pm 0.366$ & $0.766 \pm 0.332$	&  $0.220 \pm 0.308$ \\
recall	& $0.981 \pm 0.038$ 	& $0.459 \pm 0.428$ & $0.752 \pm 0.289$	&  $0.370 \pm 0.473$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{sim ECG - tachycardia} \\
\cmidrule{1-5}
length (M)    &   $910$  &    $1110$  &    $1210$   &  $1128.04 \pm 1024.98$ \\
$\mathrm{F}_1$	& $0.834 \pm 0.094$ 	& $0.428 \pm 0.092$ & $0.765 \pm 0.177$	&  $0.368 \pm 0.381$ \\
precision    & $0.861 \pm 0.115$ 	& $0.425 \pm 0.119$ & $0.751 \pm 0.267$	&  $0.305 \pm 0.344$ \\
recall	& $0.815 \pm 0.091$ 	& $0.498 \pm 0.144$ & $0.894 \pm 0.141$	&  $0.548 \pm 0.498$ \\
\cmidrule{1-5}
dataset & \multicolumn{4}{c}{random walk - linear} \\
\cmidrule{1-5}
length (M)    &   $51$  &    $21$  &    $141$   &  $161.01 \pm 80.38$ \\
$\mathrm{F}_1$	& $0.977 \pm 0.018$ 	& $0.040 \pm 0.026$ & $0.269 \pm 0.393$	&  $0.007 \pm 0.034$ \\
precision    & $0.999 \pm 0.004$ 	& $0.107 \pm 0.033$ & $0.284 \pm 0.425$	&  $0.006 \pm 0.030$ \\
recall	& $0.956 \pm 0.033$ 	& $0.027 \pm 0.023$ & $0.266 \pm 0.387$	&  $0.015 \pm 0.104$ \\
\bottomrule
\end{tabular}

==> TOF arXiv version2/latexmkrc <==
$dvipdf = 'dvipdfmx %O -o %D %S';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
    }
}


==> latexmkrc <==
$dvipdf = 'dvipdfmx %O -o %D %S';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
    }
}

